From Generic to Dedicated: A Novel Optimizer for Online Continual Learning

Online Continual Learning (OCL) requires models to learn from non-stationary data streams under a strict single-pass constraint, making them highly susceptible to catastrophic forgetting. While existing studies have explored various strategies from data, architecture, and optimization perspectives, the optimizer often directly uses generic approaches such as SGD and AdamW. In this work, we reveal a new link between optimization dynamics and OCL needs by recasting Polyak-Ruppert averaging as the engine of "plasticity" and Primal averaging as the anchor of "stability". This inspires our novel optimizer, SPIN (Stability-Plasticity INterpolation), which explicitly decouples plasticity and stability by interpolating between a fast-moving "plasticity" sequence and an adaptive "stability" sequence. We theoretically demonstrate that SPIN implicitly employs an inverse Hessian approximation, providing crucial Tikhonov regularization to damp noisy, single-sample Hessian estimates and mitigate forgetting. More importantly, SPIN can be seamlessly integrated into existing OCL methods by taking resulted gradients as input and replacing standard optimizers. Extensive experiments show that using SPIN instead of standard optimizers yields consistent and significant performance gains across multiple OCL approaches, including the challenging rehearsal-free setting and under strict memory constraints.

==> cvpr24_hparams_table.tex <==
\begin{landscape}
\scriptsize
\setlength{\LTleft}{0pt}
\setlength{\LTright}{0pt}
\begin{longtable}{p{0.09\linewidth} p{0.24\linewidth} p{0.12\linewidth} p{0.50\linewidth}}
\caption{Hyperparameters in \texttt{CCL-DC1/config/CVPR24}.}\\
\toprule
Dataset & Config file & Learner & Hyperparameters \\
\midrule
\endfirsthead
\toprule
Dataset & Config file & Learner & Hyperparameters \\
\midrule
\endhead
\midrule
\multicolumn{4}{r}{Continued on next page}\\
\endfoot
\bottomrule
\endlastfoot
cifar10 & DERPP,c10,m1000.yaml & DERPP & \texttt{optim}=AdamW; \texttt{learning\_rate}=0.0005; \texttt{momentum}=0.9; \texttt{weight\_decay}=0.0001; \texttt{n\_classes}=10; \texttt{n\_tasks}=5; \texttt{mem\_size}=1000; \texttt{mem\_batch\_size}=64; \texttt{batch\_size}=10; \texttt{nf}=64; \texttt{training\_type}=inc; \texttt{seed}=0; \texttt{derpp\_alpha}=0.2; \texttt{derpp\_beta}=1.0; \texttt{tf\_type}=partial \\
cifar10 & DERPP,c10,m500.yaml & DERPP & \texttt{optim}=AdamW; \texttt{learning\_rate}=0.0005; \texttt{momentum}=0.9; \texttt{weight\_decay}=0.0001; \texttt{n\_classes}=10; \texttt{n\_tasks}=5; \texttt{mem\_size}=500; \texttt{mem\_batch\_size}=64; \texttt{batch\_size}=10; \texttt{nf}=64; \texttt{training\_type}=inc; \texttt{seed}=0; \texttt{derpp\_alpha}=0.2; \texttt{derpp\_beta}=1.0; \texttt{tf\_type}=partial \\
cifar10 & DERPPCCLDC,c10,m1000.yaml & DERPPCCLDC & \texttt{optim}=AdamW; \texttt{learning\_rate}=0.0005; \texttt{momentum}=0.9; \texttt{weight\_decay}=0.0001; \texttt{n\_classes}=10; \texttt{n\_tasks}=5; \texttt{mem\_size}=1000; \texttt{mem\_batch\_size}=64; \texttt{batch\_size}=10; \texttt{nf}=64; \texttt{training\_type}=inc; \texttt{seed}=0; \texttt{derpp\_alpha}=0.2; \texttt{derpp\_beta}=1.0; \texttt{tf\_type}=partial; \texttt{randaug\_m}=15; \texttt{randaug\_n}=3 \\
cifar10 & DERPPCCLDC,c10,m500.yaml & DERPPCCLDC & \texttt{optim}=AdamW; \texttt{learning\_rate}=0.0005; \texttt{momentum}=0.9; \texttt{weight\_decay}=0.0001; \texttt{n\_classes}=10; \texttt{n\_tasks}=5; \texttt{mem\_size}=500; \texttt{mem\_batch\_size}=64; \texttt{batch\_size}=10; \texttt{nf}=64; \texttt{training\_type}=inc; \texttt{seed}=0; \texttt{derpp\_alpha}=0.2; \texttt{derpp\_beta}=1.0; \texttt{tf\_type}=partial; \texttt{randaug\_m}=15; \texttt{randaug\_n}=3 \\
cifar10 & ER,c10,m1000.yaml & ER & \texttt{optim}=AdamW; \texttt{learning\_rate}=0.0005; \texttt{momentum}=0; \texttt{weight\_decay}=0.0001; \texttt{n\_classes}=10; \texttt{n\_tasks}=5; \texttt{mem\_size}=1000; \texttt{mem\_batch\_size}=64; \texttt{batch\_size}=10; \texttt{nf}=64; \texttt{tf\_type}=full; \texttt{training\_type}=inc; \texttt{seed}=0 \\
cifar10 & ER,c10,m500.yaml & ER & \texttt{optim}=AdamW; \texttt{learning\_rate}=0.0005; \texttt{momentum}=0; \texttt{weight\_decay}=0.0001; \texttt{n\_classes}=10; \texttt{n\_tasks}=5; \texttt{mem\_size}=500; \texttt{mem\_batch\_size}=64; \texttt{batch\_size}=10; \texttt{nf}=64; \texttt{tf\_type}=full; \texttt{training\_type}=inc; \texttt{seed}=0 \\
cifar10 & ERACE,c10,m1000.yaml & ERACE & \texttt{optim}=AdamW; \texttt{learning\_rate}=0.0005; \texttt{momentum}=0; \texttt{weight\_decay}=0.0001; \texttt{n\_classes}=10; \texttt{n\_tasks}=5; \texttt{mem\_size}=1000; \texttt{mem\_batch\_size}=64; \texttt{batch\_size}=10; \texttt{nf}=64; \texttt{tf\_type}=partial; \texttt{training\_type}=inc; \texttt{seed}=0 \\
cifar10 & ERACE,c10,m500.yaml & ERACE & \texttt{optim}=AdamW; \texttt{learning\_rate}=0.0005; \texttt{momentum}=0; \texttt{weight\_decay}=0.0001; \texttt{n\_classes}=10; \texttt{n\_tasks}=5; \texttt{mem\_size}=500; \texttt{mem\_batch\_size}=64; \texttt{batch\_size}=10; \texttt{nf}=64; \texttt{tf\_type}=partial; \texttt{training\_type}=inc; \texttt{seed}=0 \\
cifar10 & ERACECCLDC,c10,m1000.yaml & ERACECCLDC & \texttt{optim}=AdamW; \texttt{learning\_rate}=0.0005; \texttt{momentum}=0; \texttt{weight\_decay}=0.0001; \texttt{n\_classes}=10; \texttt{n\_tasks}=5; \texttt{mem\_size}=1000; \texttt{mem\_batch\_size}=64; \texttt{batch\_size}=10; \texttt{nf}=64; \texttt{tf\_type}=partial; \texttt{training\_type}=inc; \texttt{seed}=0; \texttt{randaug\_m}=15; \texttt{randaug\_n}=3; \texttt{kd\_lambda}=1 \\
cifar10 & ERACECCLDC,c10,m500.yaml & ERACECCLDC & \texttt{optim}=AdamW; \texttt{learning\_rate}=0.0005; \texttt{momentum}=0; \texttt{weight\_decay}=0.0001; \texttt{n\_classes}=10; \texttt{n\_tasks}=5; \texttt{mem\_size}=500; \texttt{mem\_batch\_size}=64; \texttt{batch\_size}=10; \texttt{nf}=64; \texttt{tf\_type}=partial; \texttt{training\_type}=inc; \texttt{seed}=0; \texttt{randaug\_m}=15; \texttt{randaug\_n}=3; \texttt{kd\_lambda}=1 \\
cifar10 & ERCCLDC,c10,m1000.yaml & ERCCLDC & \texttt{optim}=AdamW; \texttt{learning\_rate}=0.0005; \texttt{momentum}=0; \texttt{weight\_decay}=0.0001; \texttt{n\_classes}=10; \texttt{n\_tasks}=5; \texttt{mem\_size}=1000; \texttt{mem\_batch\_size}=64; \texttt{batch\_size}=10; \texttt{nf}=64; \texttt{tf\_type}=full; \texttt{training\_type}=inc; \texttt{seed}=0; \texttt{randaug\_m}=15; \texttt{randaug\_n}=3; \texttt{kd\_lambda}=2 \\
cifar10 & ERCCLDC,c10,m500.yaml & ERCCLDC & \texttt{optim}=AdamW; \texttt{learning\_rate}=0.0005; \texttt{momentum}=0; \texttt{weight\_decay}=0.0001; \texttt{n\_classes}=10; \texttt{n\_tasks}=5; \texttt{mem\_size}=500; \texttt{mem\_batch\_size}=64; \texttt{batch\_size}=10; \texttt{nf}=64; \texttt{tf\_type}=full; \texttt{training\_type}=inc; \texttt{seed}=0; \texttt{randaug\_m}=15; \texttt{randaug\_n}=3; \texttt{kd\_lambda}=2 \\
cifar10 & GSA,c10,m1000.yaml & GSA & \texttt{optim}=AdamW; \texttt{learning\_rate}=0.0005; \texttt{momentum}=0; \texttt{weight\_decay}=0.0001; \texttt{n\_classes}=10; \texttt{n\_tasks}=5; \texttt{mem\_size}=1000; \texttt{mem\_batch\_size}=64; \texttt{batch\_size}=10; \texttt{nf}=64; \texttt{tf\_type}=partial; \texttt{training\_type}=inc; \texttt{seed}=0 \\
cifar10 & GSA,c10,m500.yaml & GSA & \texttt{optim}=AdamW; \texttt{learning\_rate}=0.0005; \texttt{momentum}=0; \texttt{weight\_decay}=0.0001; \texttt{n\_classes}=10; \texttt{n\_tasks}=5; \texttt{mem\_size}=500; \texttt{mem\_batch\_size}=64; \texttt{batch\_size}=10; \texttt{nf}=64; \texttt{tf\_type}=partial; \texttt{training\_type}=inc; \texttt{seed}=0 \\
cifar10 & GSACCLDC,c10,m1000.yaml & GSACCLDC & \texttt{optim}=AdamW; \texttt{learning\_rate}=0.0005; \texttt{momentum}=0; \texttt{weight\_decay}=0.0001; \texttt{n\_classes}=10; \texttt{n\_tasks}=5; \texttt{mem\_size}=1000; \texttt{mem\_batch\_size}=64; \texttt{batch\_size}=10; \texttt{nf}=64; \texttt{tf\_type}=partial; \texttt{training\_type}=inc; \texttt{seed}=0; \texttt{randaug\_m}=15; \texttt{randaug\_n}=3 \\
cifar10 & GSACCLDC,c10,m500.yaml & GSACCLDC & \texttt{optim}=AdamW; \texttt{learning\_rate}=0.0005; \texttt{momentum}=0; \texttt{weight\_decay}=0.0001; \texttt{n\_classes}=10; \texttt{n\_tasks}=5; \texttt{mem\_size}=500; \texttt{mem\_batch\_size}=64; \texttt{batch\_size}=10; \texttt{nf}=64; \texttt{tf\_type}=partial; \texttt{training\_type}=inc; \texttt{seed}=0; \texttt{randaug\_m}=15; \texttt{randaug\_n}=3 \\
cifar10 & OCM,c10,m1000.yaml & OCM & \texttt{optim}=AdamW; \texttt{learning\_rate}=0.001; \texttt{momentum}=0; \texttt{weight\_decay}=0; \texttt{n\_classes}=10; \texttt{n\_tasks}=5; \texttt{mem\_size}=1000; \texttt{mem\_batch\_size}=64; \texttt{batch\_size}=10; \texttt{nf}=64; \texttt{tf\_type}=full; \texttt{training\_type}=inc; \texttt{seed}=0; \texttt{proj\_dim}=128 \\
cifar10 & OCM,c10,m500.yaml & OCM & \texttt{optim}=AdamW; \texttt{learning\_rate}=0.001; \texttt{momentum}=0; \texttt{weight\_decay}=0; \texttt{n\_classes}=10; \texttt{n\_tasks}=5; \texttt{mem\_size}=500; \texttt{mem\_batch\_size}=64; \texttt{batch\_size}=10; \texttt{nf}=64; \texttt{tf\_type}=full; \texttt{training\_type}=inc; \texttt{seed}=0; \texttt{proj\_dim}=128 \\
cifar10 & OCMCCLDC,c10,m1000.yaml & OCMCCLDC & \texttt{optim}=AdamW; \texttt{learning\_rate}=0.001; \texttt{momentum}=0; \texttt{weight\_decay}=0; \texttt{n\_classes}=10; \texttt{n\_tasks}=5; \texttt{mem\_size}=1000; \texttt{mem\_batch\_size}=64; \texttt{batch\_size}=10; \texttt{nf}=64; \texttt{tf\_type}=full; \texttt{training\_type}=inc; \texttt{seed}=0; \texttt{randaug\_m}=15; \texttt{randaug\_n}=3; \texttt{kd\_lambda}=4; \texttt{proj\_dim}=128 \\
cifar10 & OCMCCLDC,c10,m500.yaml & OCMCCLDC & \texttt{optim}=AdamW; \texttt{learning\_rate}=0.001; \texttt{momentum}=0; \texttt{weight\_decay}=0; \texttt{n\_classes}=10; \texttt{n\_tasks}=5; \texttt{mem\_size}=500; \texttt{mem\_batch\_size}=64; \texttt{batch\_size}=10; \texttt{nf}=64; \texttt{tf\_type}=full; \texttt{training\_type}=inc; \texttt{seed}=0; \texttt{randaug\_m}=15; \texttt{randaug\_n}=3; \texttt{kd\_lambda}=4; \texttt{proj\_dim}=128 \\
cifar10 & ONPRO,c10,m1000.yaml & OnPro & \texttt{optim}=AdamW; \texttt{learning\_rate}=0.0005; \texttt{momentum}=0; \texttt{weight\_decay}=0.0001; \texttt{n\_classes}=10; \texttt{n\_tasks}=5; \texttt{mem\_size}=1000; \texttt{mem\_batch\_size}=64; \texttt{batch\_size}=10; \texttt{nf}=64; \texttt{tf\_type}=full; \texttt{training\_type}=inc; \texttt{seed}=0 \\
cifar10 & ONPRO,c10,m500.yaml & OnPro & \texttt{optim}=AdamW; \texttt{learning\_rate}=0.0005; \texttt{momentum}=0; \texttt{weight\_decay}=0.0001; \texttt{n\_classes}=10; \texttt{n\_tasks}=5; \texttt{mem\_size}=500; \texttt{mem\_batch\_size}=64; \texttt{batch\_size}=10; \texttt{nf}=64; \texttt{tf\_type}=full; \texttt{training\_type}=inc; \texttt{seed}=0 \\
cifar10 & ONPROCCLDC,c10,m1000.yaml & OnProCCLDC & \texttt{optim}=AdamW; \texttt{learning\_rate}=0.0005; \texttt{momentum}=0; \texttt{weight\_decay}=0.0001; \texttt{n\_classes}=10; \texttt{n\_tasks}=5; \texttt{mem\_size}=1000; \texttt{mem\_batch\_size}=64; \texttt{batch\_size}=10; \texttt{nf}=64; \texttt{tf\_type}=full; \texttt{training\_type}=inc; \texttt{seed}=0; \texttt{randaug\_m}=15; \texttt{randaug\_n}=3 \\
cifar10 & ONPROCCLDC,c10,m500.yaml & OnProCCLDC & \texttt{optim}=AdamW; \texttt{learning\_rate}=0.0005; \texttt{momentum}=0; \texttt{weight\_decay}=0.0001; \texttt{n\_classes}=10; \texttt{n\_tasks}=5; \texttt{mem\_size}=500; \texttt{mem\_batch\_size}=64; \texttt{batch\_size}=10; \texttt{nf}=64; \texttt{tf\_type}=full; \texttt{training\_type}=inc; \texttt{seed}=0; \texttt{randaug\_m}=15; \texttt{randaug\_n}=3 \\
cifar100 & DERPP,c100,m1000.yaml & DERPP & \texttt{optim}=AdamW; \texttt{learning\_rate}=0.0005; \texttt{momentum}=0.9; \texttt{weight\_decay}=0.0001; \texttt{n\_classes}=100; \texttt{n\_tasks}=10; \texttt{mem\_size}=1000; \texttt{mem\_batch\_size}=64; \texttt{batch\_size}=10; \texttt{nf}=64; \texttt{training\_type}=inc; \texttt{seed}=0; \texttt{derpp\_alpha}=0.2; \texttt{derpp\_beta}=1.0; \texttt{tf\_type}=partial \\
cifar100 & DERPP,c100,m2000.yaml & DERPP & \texttt{optim}=AdamW; \texttt{learning\_rate}=0.0005; \texttt{momentum}=0.9; \texttt{weight\_decay}=0.0001; \texttt{n\_classes}=100; \texttt{n\_tasks}=10; \texttt{mem\_size}=2000; \texttt{mem\_batch\_size}=64; \texttt{batch\_size}=10; \texttt{nf}=64; \texttt{training\_type}=inc; \texttt{seed}=0; \texttt{derpp\_alpha}=0.2; \texttt{derpp\_beta}=1.0; \texttt{tf\_type}=partial \\
cifar100 & DERPP,c100,m5000.yaml & DERPP & \texttt{optim}=AdamW; \texttt{learning\_rate}=0.0005; \texttt{momentum}=0.9; \texttt{weight\_decay}=0.0001; \texttt{n\_classes}=100; \texttt{n\_tasks}=10; \texttt{mem\_size}=5000; \texttt{mem\_batch\_size}=64; \texttt{batch\_size}=10; \texttt{nf}=64; \texttt{training\_type}=inc; \texttt{seed}=0; \texttt{derpp\_alpha}=0.2; \texttt{derpp\_beta}=1.0; \texttt{tf\_type}=partial \\
cifar100 & DERPPCCLDC,c100,m1000.yaml & DERPPCCLDC & \texttt{optim}=AdamW; \texttt{learning\_rate}=0.0005; \texttt{momentum}=0.9; \texttt{weight\_decay}=0.0001; \texttt{n\_classes}=100; \texttt{n\_tasks}=10; \texttt{mem\_size}=1000; \texttt{mem\_batch\_size}=64; \texttt{batch\_size}=10; \texttt{nf}=64; \texttt{training\_type}=inc; \texttt{seed}=0; \texttt{derpp\_alpha}=0.2; \texttt{derpp\_beta}=1.0; \texttt{tf\_type}=partial; \texttt{randaug\_m}=15; \texttt{randaug\_n}=3 \\
cifar100 & DERPPCCLDC,c100,m2000.yaml & DERPPCCLDC & \texttt{optim}=AdamW; \texttt{learning\_rate}=0.0005; \texttt{momentum}=0.9; \texttt{weight\_decay}=0.0001; \texttt{n\_classes}=100; \texttt{n\_tasks}=10; \texttt{mem\_size}=2000; \texttt{mem\_batch\_size}=64; \texttt{batch\_size}=10; \texttt{nf}=64; \texttt{training\_type}=inc; \texttt{seed}=0; \texttt{derpp\_alpha}=0.2; \texttt{derpp\_beta}=1.0; \texttt{tf\_type}=partial; \texttt{randaug\_m}=15; \texttt{randaug\_n}=3 \\
cifar100 & DERPPCCLDC,c100,m5000.yaml & DERPPCCLDC & \texttt{optim}=AdamW; \texttt{learning\_rate}=0.0005; \texttt{momentum}=0.9; \texttt{weight\_decay}=0.0001; \texttt{n\_classes}=100; \texttt{n\_tasks}=10; \texttt{mem\_size}=5000; \texttt{mem\_batch\_size}=64; \texttt{batch\_size}=10; \texttt{nf}=64; \texttt{training\_type}=inc; \texttt{seed}=0; \texttt{derpp\_alpha}=0.2; \texttt{derpp\_beta}=1.0; \texttt{tf\_type}=partial; \texttt{randaug\_m}=15; \texttt{randaug\_n}=3 \\
cifar100 & ER,c100,m1000.yaml & ER & \texttt{optim}=AdamW; \texttt{learning\_rate}=0.0005; \texttt{momentum}=0; \texttt{weight\_decay}=0.0001; \texttt{n\_classes}=100; \texttt{n\_tasks}=10; \texttt{mem\_size}=1000; \texttt{mem\_batch\_size}=64; \texttt{batch\_size}=10; \texttt{nf}=64; \texttt{tf\_type}=full; \texttt{training\_type}=inc; \texttt{seed}=0 \\
cifar100 & ER,c100,m2000.yaml & ER & \texttt{optim}=spin; \texttt{learning\_rate}=0.0005; \texttt{momentum}=0; \texttt{weight\_decay}=0.0001; \texttt{n\_classes}=100; \texttt{n\_tasks}=10; \texttt{mem\_size}=2000; \texttt{mem\_batch\_size}=64; \texttt{batch\_size}=10; \texttt{nf}=64; \texttt{tf\_type}=full; \texttt{training\_type}=inc; \texttt{seed}=1995 \\
cifar100 & ER,c100,m5000.yaml & ER & \texttt{optim}=AdamW; \texttt{learning\_rate}=0.0005; \texttt{momentum}=0; \texttt{weight\_decay}=0.0001; \texttt{n\_classes}=100; \texttt{n\_tasks}=10; \texttt{mem\_size}=5000; \texttt{mem\_batch\_size}=64; \texttt{batch\_size}=10; \texttt{nf}=64; \texttt{tf\_type}=full; \texttt{training\_type}=inc; \texttt{seed}=0 \\
cifar100 & ERACE,c100,m1000.yaml & ERACE & \texttt{optim}=AdamW; \texttt{learning\_rate}=0.0005; \texttt{momentum}=0; \texttt{weight\_decay}=0.0001; \texttt{n\_classes}=100; \texttt{n\_tasks}=10; \texttt{mem\_size}=1000; \texttt{mem\_batch\_size}=64; \texttt{batch\_size}=10; \texttt{nf}=64; \texttt{tf\_type}=partial; \texttt{training\_type}=inc; \texttt{seed}=0 \\
cifar100 & ERACE,c100,m2000.yaml & ERACE & \texttt{optim}=AdamW; \texttt{learning\_rate}=0.0005; \texttt{momentum}=0; \texttt{weight\_decay}=0.0001; \texttt{n\_classes}=100; \texttt{n\_tasks}=10; \texttt{mem\_size}=2000; \texttt{mem\_batch\_size}=64; \texttt{batch\_size}=10; \texttt{nf}=64; \texttt{tf\_type}=partial; \texttt{training\_type}=inc; \texttt{seed}=0 \\
cifar100 & ERACE,c100,m5000.yaml & ERACE & \texttt{optim}=AdamW; \texttt{learning\_rate}=0.0005; \texttt{momentum}=0; \texttt{weight\_decay}=0.0001; \texttt{n\_classes}=100; \texttt{n\_tasks}=10; \texttt{mem\_size}=5000; \texttt{mem\_batch\_size}=64; \texttt{batch\_size}=10; \texttt{nf}=64; \texttt{tf\_type}=partial; \texttt{training\_type}=inc; \texttt{seed}=0 \\
cifar100 & ERACECCLDC,c100,m1000.yaml & ERACECCLDC & \texttt{optim}=AdamW; \texttt{learning\_rate}=0.0005; \texttt{momentum}=0; \texttt{weight\_decay}=0.0001; \texttt{n\_classes}=100; \texttt{n\_tasks}=10; \texttt{mem\_size}=1000; \texttt{mem\_batch\_size}=64; \texttt{batch\_size}=10; \texttt{nf}=64; \texttt{tf\_type}=partial; \texttt{training\_type}=inc; \texttt{seed}=0; \texttt{randaug\_m}=15; \texttt{randaug\_n}=3; \texttt{kd\_lambda}=1 \\
cifar100 & ERACECCLDC,c100,m2000.yaml & ERACECCLDC & \texttt{optim}=AdamW; \texttt{learning\_rate}=0.0005; \texttt{momentum}=0; \texttt{weight\_decay}=0.0001; \texttt{n\_classes}=100; \texttt{n\_tasks}=10; \texttt{mem\_size}=2000; \texttt{mem\_batch\_size}=64; \texttt{batch\_size}=10; \texttt{nf}=64; \texttt{tf\_type}=partial; \texttt{training\_type}=inc; \texttt{seed}=0; \texttt{randaug\_m}=15; \texttt{randaug\_n}=3; \texttt{kd\_lambda}=1 \\
cifar100 & ERACECCLDC,c100,m5000.yaml & ERACECCLDC & \texttt{optim}=AdamW; \texttt{learning\_rate}=0.0005; \texttt{momentum}=0; \texttt{weight\_decay}=0.0001; \texttt{n\_classes}=100; \texttt{n\_tasks}=10; \texttt{mem\_size}=5000; \texttt{mem\_batch\_size}=64; \texttt{batch\_size}=10; \texttt{nf}=64; \texttt{tf\_type}=partial; \texttt{training\_type}=inc; \texttt{seed}=0; \texttt{randaug\_m}=15; \texttt{randaug\_n}=3; \texttt{kd\_lambda}=1 \\
cifar100 & ERCCLDC,c100,m1000.yaml & ERCCLDC & \texttt{optim}=AdamW; \texttt{learning\_rate}=0.0005; \texttt{momentum}=0; \texttt{weight\_decay}=0.0001; \texttt{n\_classes}=100; \texttt{n\_tasks}=10; \texttt{mem\_size}=1000; \texttt{mem\_batch\_size}=64; \texttt{batch\_size}=10; \texttt{nf}=64; \texttt{tf\_type}=full; \texttt{training\_type}=inc; \texttt{seed}=0; \texttt{randaug\_m}=15; \texttt{randaug\_n}=3; \texttt{kd\_lambda}=2 \\
cifar100 & ERCCLDC,c100,m2000.yaml & ERCCLDC & \texttt{optim}=AdamW; \texttt{learning\_rate}=0.0005; \texttt{momentum}=0; \texttt{weight\_decay}=0.0001; \texttt{n\_classes}=100; \texttt{n\_tasks}=10; \texttt{mem\_size}=2000; \texttt{mem\_batch\_size}=64; \texttt{batch\_size}=10; \texttt{nf}=64; \texttt{tf\_type}=full; \texttt{training\_type}=inc; \texttt{seed}=0; \texttt{randaug\_m}=15; \texttt{randaug\_n}=3; \texttt{kd\_lambda}=2 \\
cifar100 & ERCCLDC,c100,m5000.yaml & ERCCLDC & \texttt{optim}=AdamW; \texttt{learning\_rate}=0.0005; \texttt{momentum}=0; \texttt{weight\_decay}=0.0001; \texttt{n\_classes}=100; \texttt{n\_tasks}=10; \texttt{mem\_size}=5000; \texttt{mem\_batch\_size}=64; \texttt{batch\_size}=10; \texttt{nf}=64; \texttt{tf\_type}=full; \texttt{training\_type}=inc; \texttt{seed}=0; \texttt{randaug\_m}=15; \texttt{randaug\_n}=3; \texttt{kd\_lambda}=2 \\
cifar100 & GSA,c100,m1000.yaml & GSA & \texttt{optim}=spin\_sgd; \texttt{learning\_rate}=0.01; \texttt{momentum}=0.0; \texttt{weight\_decay}=0.0001; \texttt{n\_classes}=100; \texttt{n\_tasks}=10; \texttt{mem\_size}=30000; \texttt{mem\_batch\_size}=64; \texttt{batch\_size}=10; \texttt{nf}=64; \texttt{tf\_type}=partial; \texttt{training\_type}=inc; \texttt{seed}=0; \texttt{backbone}=resnet18 \\
cifar100 & GSA,c100,m2000.yaml & GSA & \texttt{optim}=AdamW; \texttt{learning\_rate}=0.0005; \texttt{momentum}=0; \texttt{weight\_decay}=0.0001; \texttt{n\_classes}=100; \texttt{n\_tasks}=10; \texttt{mem\_size}=2000; \texttt{mem\_batch\_size}=64; \texttt{batch\_size}=10; \texttt{nf}=64; \texttt{tf\_type}=partial; \texttt{training\_type}=inc; \texttt{seed}=0 \\
cifar100 & GSA,c100,m5000.yaml & GSA & \texttt{optim}=AdamW; \texttt{learning\_rate}=0.0005; \texttt{momentum}=0; \texttt{weight\_decay}=0.0001; \texttt{n\_classes}=100; \texttt{n\_tasks}=10; \texttt{mem\_size}=5000; \texttt{mem\_batch\_size}=64; \texttt{batch\_size}=10; \texttt{nf}=64; \texttt{tf\_type}=partial; \texttt{training\_type}=inc; \texttt{seed}=0 \\
cifar100 & GSACCLDC,c100,m1000.yaml & GSACCLDC & \texttt{optim}=AdamW; \texttt{learning\_rate}=0.0005; \texttt{momentum}=0; \texttt{weight\_decay}=0.0001; \texttt{n\_classes}=100; \texttt{n\_tasks}=10; \texttt{mem\_size}=1000; \texttt{mem\_batch\_size}=64; \texttt{batch\_size}=10; \texttt{nf}=64; \texttt{tf\_type}=partial; \texttt{training\_type}=inc; \texttt{seed}=0; \texttt{randaug\_m}=15; \texttt{randaug\_n}=3 \\
cifar100 & GSACCLDC,c100,m2000.yaml & GSACCLDC & \texttt{optim}=AdamW; \texttt{learning\_rate}=0.0005; \texttt{momentum}=0; \texttt{weight\_decay}=0.0001; \texttt{n\_classes}=100; \texttt{n\_tasks}=10; \texttt{mem\_size}=2000; \texttt{mem\_batch\_size}=64; \texttt{batch\_size}=10; \texttt{nf}=64; \texttt{tf\_type}=partial; \texttt{training\_type}=inc; \texttt{seed}=0; \texttt{randaug\_m}=15; \texttt{randaug\_n}=3 \\
cifar100 & GSACCLDC,c100,m5000.yaml & GSACCLDC & \texttt{optim}=AdamW; \texttt{learning\_rate}=0.0005; \texttt{momentum}=0; \texttt{weight\_decay}=0.0001; \texttt{n\_classes}=100; \texttt{n\_tasks}=10; \texttt{mem\_size}=5000; \texttt{mem\_batch\_size}=64; \texttt{batch\_size}=10; \texttt{nf}=64; \texttt{tf\_type}=partial; \texttt{training\_type}=inc; \texttt{seed}=0; \texttt{randaug\_m}=15; \texttt{randaug\_n}=3 \\
cifar100 & OCM,c100,m1000.yaml & OCM & \texttt{optim}=AdamW; \texttt{learning\_rate}=0.001; \texttt{momentum}=0; \texttt{weight\_decay}=0; \texttt{n\_classes}=100; \texttt{n\_tasks}=10; \texttt{mem\_size}=1000; \texttt{mem\_batch\_size}=64; \texttt{batch\_size}=10; \texttt{nf}=64; \texttt{tf\_type}=full; \texttt{training\_type}=inc; \texttt{seed}=0; \texttt{proj\_dim}=128 \\
cifar100 & OCM,c100,m2000.yaml & OCM & \texttt{optim}=AdamW; \texttt{learning\_rate}=0.001; \texttt{momentum}=0; \texttt{weight\_decay}=0; \texttt{n\_classes}=100; \texttt{n\_tasks}=10; \texttt{mem\_size}=2000; \texttt{mem\_batch\_size}=64; \texttt{batch\_size}=10; \texttt{nf}=64; \texttt{tf\_type}=full; \texttt{training\_type}=inc; \texttt{seed}=0; \texttt{proj\_dim}=128 \\
cifar100 & OCM,c100,m5000.yaml & OCM & \texttt{optim}=AdamW; \texttt{learning\_rate}=0.001; \texttt{momentum}=0; \texttt{weight\_decay}=0; \texttt{n\_classes}=100; \texttt{n\_tasks}=10; \texttt{mem\_size}=5000; \texttt{mem\_batch\_size}=64; \texttt{batch\_size}=10; \texttt{nf}=64; \texttt{tf\_type}=full; \texttt{training\_type}=inc; \texttt{seed}=0; \texttt{proj\_dim}=128 \\
cifar100 & OCMCCLDC,c100,m1000.yaml & OCMCCLDC & \texttt{optim}=AdamW; \texttt{learning\_rate}=0.001; \texttt{momentum}=0; \texttt{weight\_decay}=0; \texttt{n\_classes}=100; \texttt{n\_tasks}=10; \texttt{mem\_size}=1000; \texttt{mem\_batch\_size}=64; \texttt{batch\_size}=10; \texttt{nf}=64; \texttt{tf\_type}=full; \texttt{training\_type}=inc; \texttt{seed}=0; \texttt{randaug\_m}=15; \texttt{randaug\_n}=3; \texttt{kd\_lambda}=4; \texttt{proj\_dim}=128 \\
cifar100 & OCMCCLDC,c100,m2000.yaml & OCMCCLDC & \texttt{optim}=AdamW; \texttt{learning\_rate}=0.001; \texttt{momentum}=0; \texttt{weight\_decay}=0; \texttt{n\_classes}=100; \texttt{n\_tasks}=10; \texttt{mem\_size}=2000; \texttt{mem\_batch\_size}=64; \texttt{batch\_size}=10; \texttt{nf}=64; \texttt{tf\_type}=full; \texttt{training\_type}=inc; \texttt{seed}=0; \texttt{randaug\_m}=15; \texttt{randaug\_n}=3; \texttt{kd\_lambda}=4; \texttt{proj\_dim}=128 \\
cifar100 & OCMCCLDC,c100,m5000.yaml & OCMCCLDC & \texttt{optim}=AdamW; \texttt{learning\_rate}=0.001; \texttt{momentum}=0; \texttt{weight\_decay}=0; \texttt{n\_classes}=100; \texttt{n\_tasks}=10; \texttt{mem\_size}=5000; \texttt{mem\_batch\_size}=64; \texttt{batch\_size}=10; \texttt{nf}=64; \texttt{tf\_type}=full; \texttt{training\_type}=inc; \texttt{seed}=0; \texttt{randaug\_m}=15; \texttt{randaug\_n}=3; \texttt{kd\_lambda}=4; \texttt{proj\_dim}=128 \\
cifar100 & ONPRO,c100,m1000.yaml & OnPro & \texttt{optim}=AdamW; \texttt{learning\_rate}=0.0005; \texttt{momentum}=0; \texttt{weight\_decay}=0.0001; \texttt{n\_classes}=100; \texttt{n\_tasks}=10; \texttt{mem\_size}=1000; \texttt{mem\_batch\_size}=64; \texttt{batch\_size}=10; \texttt{nf}=64; \texttt{tf\_type}=full; \texttt{training\_type}=inc; \texttt{seed}=0 \\
cifar100 & ONPRO,c100,m2000.yaml & OnPro & \texttt{optim}=AdamW; \texttt{learning\_rate}=0.0005; \texttt{momentum}=0; \texttt{weight\_decay}=0.0001; \texttt{n\_classes}=100; \texttt{n\_tasks}=10; \texttt{mem\_size}=2000; \texttt{mem\_batch\_size}=64; \texttt{batch\_size}=10; \texttt{nf}=64; \texttt{tf\_type}=full; \texttt{training\_type}=inc; \texttt{seed}=0 \\
cifar100 & ONPRO,c100,m5000.yaml & OnPro & \texttt{optim}=AdamW; \texttt{learning\_rate}=0.0005; \texttt{momentum}=0; \texttt{weight\_decay}=0.0001; \texttt{n\_classes}=100; \texttt{n\_tasks}=10; \texttt{mem\_size}=5000; \texttt{mem\_batch\_size}=64; \texttt{batch\_size}=10; \texttt{nf}=64; \texttt{tf\_type}=full; \texttt{training\_type}=inc; \texttt{seed}=0 \\
cifar100 & ONPROCCLDC,c100,m1000.yaml & OnProCCLDC & \texttt{optim}=AdamW; \texttt{learning\_rate}=0.0005; \texttt{momentum}=0; \texttt{weight\_decay}=0.0001; \texttt{n\_classes}=100; \texttt{n\_tasks}=10; \texttt{mem\_size}=1000; \texttt{mem\_batch\_size}=64; \texttt{batch\_size}=10; \texttt{nf}=64; \texttt{tf\_type}=full; \texttt{training\_type}=inc; \texttt{seed}=0; \texttt{randaug\_m}=15; \texttt{randaug\_n}=3 \\
cifar100 & ONPROCCLDC,c100,m2000.yaml & OnProCCLDC & \texttt{optim}=AdamW; \texttt{learning\_rate}=0.0005; \texttt{momentum}=0; \texttt{weight\_decay}=0.0001; \texttt{n\_classes}=100; \texttt{n\_tasks}=10; \texttt{mem\_size}=2000; \texttt{mem\_batch\_size}=64; \texttt{batch\_size}=10; \texttt{nf}=64; \texttt{tf\_type}=full; \texttt{training\_type}=inc; \texttt{seed}=0; \texttt{randaug\_m}=15; \texttt{randaug\_n}=3 \\
cifar100 & ONPROCCLDC,c100,m5000.yaml & OnProCCLDC & \texttt{optim}=AdamW; \texttt{learning\_rate}=0.0005; \texttt{momentum}=0; \texttt{weight\_decay}=0.0001; \texttt{n\_classes}=100; \texttt{n\_tasks}=10; \texttt{mem\_size}=5000; \texttt{mem\_batch\_size}=64; \texttt{batch\_size}=10; \texttt{nf}=64; \texttt{tf\_type}=full; \texttt{training\_type}=inc; \texttt{seed}=0; \texttt{randaug\_m}=15; \texttt{randaug\_n}=3 \\
imagenet100 & DERPP,in100,m5000.yaml & DERPP & \texttt{optim}=AdamW; \texttt{learning\_rate}=0.0005; \texttt{momentum}=0.9; \texttt{weight\_decay}=0.0001; \texttt{img\_size}=224; \texttt{n\_classes}=100; \texttt{n\_tasks}=10; \texttt{mem\_size}=5000; \texttt{mem\_batch\_size}=64; \texttt{batch\_size}=10; \texttt{nf}=64; \texttt{training\_type}=inc; \texttt{seed}=0; \texttt{derpp\_alpha}=0.2; \texttt{derpp\_beta}=1.0; \texttt{tf\_type}=partial \\
imagenet100 & DERPPCCLDC,in100,m5000.yaml & DERPPCCLDC & \texttt{optim}=AdamW; \texttt{learning\_rate}=0.0005; \texttt{momentum}=0.9; \texttt{weight\_decay}=0.0001; \texttt{img\_size}=224; \texttt{n\_classes}=100; \texttt{n\_tasks}=10; \texttt{mem\_size}=5000; \texttt{mem\_batch\_size}=64; \texttt{batch\_size}=10; \texttt{nf}=64; \texttt{training\_type}=inc; \texttt{seed}=0; \texttt{derpp\_alpha}=0.2; \texttt{derpp\_beta}=1.0; \texttt{tf\_type}=partial; \texttt{randaug\_m}=11; \texttt{randaug\_n}=3 \\
imagenet100 & ER,in100,m5000.yaml & ER & \texttt{optim}=AdamW; \texttt{learning\_rate}=0.0005; \texttt{momentum}=0; \texttt{weight\_decay}=0.0001; \texttt{img\_size}=224; \texttt{n\_classes}=100; \texttt{n\_tasks}=10; \texttt{mem\_size}=5000; \texttt{mem\_batch\_size}=64; \texttt{batch\_size}=10; \texttt{nf}=64; \texttt{tf\_type}=full; \texttt{training\_type}=inc; \texttt{seed}=0 \\
imagenet100 & ERACE,in100,m5000.yaml & ERACE & \texttt{optim}=AdamW; \texttt{learning\_rate}=0.0005; \texttt{momentum}=0; \texttt{weight\_decay}=0.0001; \texttt{img\_size}=224; \texttt{n\_classes}=100; \texttt{n\_tasks}=10; \texttt{mem\_size}=5000; \texttt{mem\_batch\_size}=64; \texttt{batch\_size}=10; \texttt{nf}=64; \texttt{tf\_type}=partial; \texttt{training\_type}=inc; \texttt{seed}=0 \\
imagenet100 & ERACECCLDC,in100,m5000.yaml & ERACECCLDC & \texttt{optim}=AdamW; \texttt{learning\_rate}=0.0005; \texttt{momentum}=0; \texttt{weight\_decay}=0.0001; \texttt{img\_size}=224; \texttt{n\_classes}=100; \texttt{n\_tasks}=10; \texttt{mem\_size}=5000; \texttt{mem\_batch\_size}=64; \texttt{batch\_size}=10; \texttt{nf}=64; \texttt{tf\_type}=partial; \texttt{training\_type}=inc; \texttt{seed}=0; \texttt{randaug\_m}=11; \texttt{randaug\_n}=3; \texttt{kd\_lambda}=1 \\
imagenet100 & ERCCLDC,in100,m5000.yaml & ERCCLDC & \texttt{optim}=AdamW; \texttt{learning\_rate}=0.0005; \texttt{momentum}=0; \texttt{weight\_decay}=0.0001; \texttt{img\_size}=224; \texttt{n\_classes}=100; \texttt{n\_tasks}=10; \texttt{mem\_size}=5000; \texttt{mem\_batch\_size}=64; \texttt{batch\_size}=10; \texttt{nf}=64; \texttt{tf\_type}=full; \texttt{training\_type}=inc; \texttt{seed}=0; \texttt{randaug\_m}=11; \texttt{randaug\_n}=3; \texttt{kd\_lambda}=2 \\
imagenet100 & GSA,in100,m5000.yaml & GSA & \texttt{optim}=AdamW; \texttt{learning\_rate}=0.0005; \texttt{momentum}=0; \texttt{weight\_decay}=0.0001; \texttt{img\_size}=224; \texttt{n\_classes}=100; \texttt{n\_tasks}=10; \texttt{mem\_size}=5000; \texttt{mem\_batch\_size}=64; \texttt{batch\_size}=10; \texttt{nf}=64; \texttt{tf\_type}=partial; \texttt{training\_type}=inc; \texttt{seed}=0 \\
imagenet100 & GSACCLDC,in100,m5000.yaml & GSACCLDC & \texttt{optim}=AdamW; \texttt{learning\_rate}=0.0005; \texttt{momentum}=0; \texttt{weight\_decay}=0.0001; \texttt{img\_size}=224; \texttt{n\_classes}=100; \texttt{n\_tasks}=10; \texttt{mem\_size}=5000; \texttt{mem\_batch\_size}=64; \texttt{batch\_size}=10; \texttt{nf}=64; \texttt{tf\_type}=partial; \texttt{training\_type}=inc; \texttt{seed}=0; \texttt{randaug\_m}=11; \texttt{randaug\_n}=3 \\
imagenet100 & OCM,in100,m5000.yaml & OCM & \texttt{optim}=AdamW; \texttt{learning\_rate}=0.001; \texttt{momentum}=0; \texttt{weight\_decay}=0; \texttt{img\_size}=224; \texttt{n\_classes}=100; \texttt{n\_tasks}=10; \texttt{mem\_size}=5000; \texttt{mem\_batch\_size}=64; \texttt{batch\_size}=10; \texttt{nf}=64; \texttt{tf\_type}=full; \texttt{training\_type}=inc; \texttt{seed}=0; \texttt{proj\_dim}=128 \\
imagenet100 & OCMCCLDC,in100,m5000.yaml & OCMCCLDC & \texttt{optim}=AdamW; \texttt{learning\_rate}=0.001; \texttt{momentum}=0; \texttt{weight\_decay}=0; \texttt{img\_size}=224; \texttt{n\_classes}=100; \texttt{n\_tasks}=10; \texttt{mem\_size}=5000; \texttt{mem\_batch\_size}=64; \texttt{batch\_size}=10; \texttt{nf}=64; \texttt{tf\_type}=full; \texttt{training\_type}=inc; \texttt{seed}=0; \texttt{randaug\_m}=11; \texttt{randaug\_n}=3; \texttt{kd\_lambda}=4; \texttt{proj\_dim}=128 \\
imagenet100 & ONPRO,in100,m5000.yaml & OnPro & \texttt{optim}=AdamW; \texttt{learning\_rate}=0.0005; \texttt{momentum}=0; \texttt{weight\_decay}=0.0001; \texttt{img\_size}=224; \texttt{n\_classes}=100; \texttt{n\_tasks}=10; \texttt{mem\_size}=5000; \texttt{mem\_batch\_size}=64; \texttt{batch\_size}=10; \texttt{nf}=64; \texttt{tf\_type}=full; \texttt{training\_type}=inc; \texttt{seed}=0 \\
imagenet100 & ONPROCCLDC,in100,m5000.yaml & OnProCCLDC & \texttt{optim}=AdamW; \texttt{learning\_rate}=0.0005; \texttt{momentum}=0; \texttt{weight\_decay}=0.0001; \texttt{img\_size}=224; \texttt{n\_classes}=100; \texttt{n\_tasks}=10; \texttt{mem\_size}=5000; \texttt{mem\_batch\_size}=64; \texttt{batch\_size}=10; \texttt{nf}=64; \texttt{tf\_type}=full; \texttt{training\_type}=inc; \texttt{seed}=0; \texttt{randaug\_m}=11; \texttt{randaug\_n}=3 \\
landmarks & ER,landmarks,m10000mbs200sbs64ER\_Landmarks\_50T.yaml & ER & \texttt{data\_root\_dir}=/home/wuyongyi/google-landmark; \texttt{img\_size}=224; \texttt{epochs}=1; \texttt{n\_tasks}=50; \texttt{batch\_size}=64; \texttt{buffer}=reservoir; \texttt{mem\_size}=10000; \texttt{mem\_iters}=1; \texttt{optim}=SGD; \texttt{learning\_rate}=0.03; \texttt{momentum}=0; \texttt{weight\_decay}=0.0001; \texttt{head}=mlp; \texttt{nf}=64; \texttt{tensorboard}=True; \texttt{verbose}=True; \texttt{tag}=ER\_Landmarks\_50T; \texttt{n\_classes}=87616; \texttt{mem\_batch\_size}=64; \texttt{tf\_type}=full; \texttt{training\_type}=inc; \texttt{seed}=0 \\
tiny & DERPP,tiny,m10000.yaml & DERPP & \texttt{optim}=AdamW; \texttt{learning\_rate}=0.0005; \texttt{momentum}=0.9; \texttt{weight\_decay}=0.0001; \texttt{img\_size}=64; \texttt{dim\_in}=2048; \texttt{n\_classes}=200; \texttt{n\_tasks}=100; \texttt{mem\_size}=10000; \texttt{mem\_batch\_size}=64; \texttt{batch\_size}=10; \texttt{nf}=64; \texttt{training\_type}=inc; \texttt{seed}=0; \texttt{derpp\_alpha}=0.2; \texttt{derpp\_beta}=1.0; \texttt{tf\_type}=partial \\
tiny & DERPP,tiny,m2000.yaml & DERPP & \texttt{optim}=AdamW; \texttt{learning\_rate}=0.0005; \texttt{momentum}=0.9; \texttt{weight\_decay}=0.0001; \texttt{img\_size}=64; \texttt{dim\_in}=2048; \texttt{n\_classes}=200; \texttt{n\_tasks}=100; \texttt{mem\_size}=2000; \texttt{mem\_batch\_size}=64; \texttt{batch\_size}=10; \texttt{nf}=64; \texttt{training\_type}=inc; \texttt{seed}=0; \texttt{derpp\_alpha}=0.2; \texttt{derpp\_beta}=1.0; \texttt{tf\_type}=partial \\
tiny & DERPP,tiny,m5000.yaml & DERPP & \texttt{optim}=AdamW; \texttt{learning\_rate}=0.0005; \texttt{momentum}=0.9; \texttt{weight\_decay}=0.0001; \texttt{img\_size}=64; \texttt{dim\_in}=2048; \texttt{n\_classes}=200; \texttt{n\_tasks}=100; \texttt{mem\_size}=5000; \texttt{mem\_batch\_size}=64; \texttt{batch\_size}=10; \texttt{nf}=64; \texttt{training\_type}=inc; \texttt{seed}=0; \texttt{derpp\_alpha}=0.2; \texttt{derpp\_beta}=1.0; \texttt{tf\_type}=partial \\
tiny & DERPPCCLDC,tiny,m10000.yaml & DERPPCCLDC & \texttt{optim}=AdamW; \texttt{learning\_rate}=0.0005; \texttt{momentum}=0.9; \texttt{weight\_decay}=0.0001; \texttt{img\_size}=64; \texttt{dim\_in}=2048; \texttt{n\_classes}=200; \texttt{n\_tasks}=100; \texttt{mem\_size}=10000; \texttt{mem\_batch\_size}=64; \texttt{batch\_size}=10; \texttt{nf}=64; \texttt{training\_type}=inc; \texttt{seed}=0; \texttt{derpp\_alpha}=0.2; \texttt{derpp\_beta}=1.0; \texttt{tf\_type}=partial; \texttt{randaug\_m}=11; \texttt{randaug\_n}=1 \\
tiny & DERPPCCLDC,tiny,m2000.yaml & DERPPCCLDC & \texttt{optim}=AdamW; \texttt{learning\_rate}=0.0005; \texttt{momentum}=0.9; \texttt{weight\_decay}=0.0001; \texttt{img\_size}=64; \texttt{dim\_in}=2048; \texttt{n\_classes}=200; \texttt{n\_tasks}=100; \texttt{mem\_size}=2000; \texttt{mem\_batch\_size}=64; \texttt{batch\_size}=10; \texttt{nf}=64; \texttt{training\_type}=inc; \texttt{seed}=0; \texttt{derpp\_alpha}=0.2; \texttt{derpp\_beta}=1.0; \texttt{tf\_type}=partial; \texttt{randaug\_m}=11; \texttt{randaug\_n}=1 \\
tiny & DERPPCCLDC,tiny,m5000.yaml & DERPPCCLDC & \texttt{optim}=AdamW; \texttt{learning\_rate}=0.0005; \texttt{momentum}=0.9; \texttt{weight\_decay}=0.0001; \texttt{img\_size}=64; \texttt{dim\_in}=2048; \texttt{n\_classes}=200; \texttt{n\_tasks}=100; \texttt{mem\_size}=5000; \texttt{mem\_batch\_size}=64; \texttt{batch\_size}=10; \texttt{nf}=64; \texttt{training\_type}=inc; \texttt{seed}=0; \texttt{derpp\_alpha}=0.2; \texttt{derpp\_beta}=1.0; \texttt{tf\_type}=partial; \texttt{randaug\_m}=11; \texttt{randaug\_n}=1 \\
tiny & ER,tiny,m10000.yaml & ER & \texttt{optim}=AdamW; \texttt{learning\_rate}=0.0005; \texttt{momentum}=0; \texttt{weight\_decay}=0.0001; \texttt{img\_size}=64; \texttt{dim\_in}=2048; \texttt{n\_classes}=200; \texttt{n\_tasks}=100; \texttt{mem\_size}=10000; \texttt{mem\_batch\_size}=64; \texttt{batch\_size}=10; \texttt{nf}=64; \texttt{tf\_type}=full; \texttt{training\_type}=inc; \texttt{seed}=0 \\
tiny & ER,tiny,m2000.yaml & ER & \texttt{optim}=AdamW; \texttt{learning\_rate}=0.0005; \texttt{momentum}=0; \texttt{weight\_decay}=0.0001; \texttt{img\_size}=64; \texttt{dim\_in}=2048; \texttt{n\_classes}=200; \texttt{n\_tasks}=100; \texttt{mem\_size}=2000; \texttt{mem\_batch\_size}=64; \texttt{batch\_size}=10; \texttt{nf}=64; \texttt{tf\_type}=full; \texttt{training\_type}=inc; \texttt{seed}=0 \\
tiny & ER,tiny,m5000.yaml & ER & \texttt{optim}=AdamW; \texttt{learning\_rate}=0.0005; \texttt{momentum}=0; \texttt{weight\_decay}=0.0001; \texttt{img\_size}=64; \texttt{dim\_in}=2048; \texttt{n\_classes}=200; \texttt{n\_tasks}=100; \texttt{mem\_size}=5000; \texttt{mem\_batch\_size}=64; \texttt{batch\_size}=10; \texttt{nf}=64; \texttt{tf\_type}=full; \texttt{training\_type}=inc; \texttt{seed}=0 \\
tiny & ERACE,tiny,m10000.yaml & ERACE & \texttt{optim}=AdamW; \texttt{learning\_rate}=0.0005; \texttt{momentum}=0; \texttt{weight\_decay}=0.0001; \texttt{img\_size}=64; \texttt{dim\_in}=2048; \texttt{n\_classes}=200; \texttt{n\_tasks}=100; \texttt{mem\_size}=10000; \texttt{mem\_batch\_size}=64; \texttt{batch\_size}=10; \texttt{nf}=64; \texttt{tf\_type}=partial; \texttt{training\_type}=inc; \texttt{seed}=0 \\
tiny & ERACE,tiny,m2000.yaml & ERACE & \texttt{optim}=AdamW; \texttt{learning\_rate}=0.0005; \texttt{momentum}=0; \texttt{weight\_decay}=0.0001; \texttt{img\_size}=64; \texttt{dim\_in}=2048; \texttt{n\_classes}=200; \texttt{n\_tasks}=100; \texttt{mem\_size}=2000; \texttt{mem\_batch\_size}=64; \texttt{batch\_size}=10; \texttt{nf}=64; \texttt{tf\_type}=partial; \texttt{training\_type}=inc; \texttt{seed}=0 \\
tiny & ERACE,tiny,m5000.yaml & ERACE & \texttt{optim}=AdamW; \texttt{learning\_rate}=0.0005; \texttt{momentum}=0; \texttt{weight\_decay}=0.0001; \texttt{img\_size}=64; \texttt{dim\_in}=2048; \texttt{n\_classes}=200; \texttt{n\_tasks}=100; \texttt{mem\_size}=5000; \texttt{mem\_batch\_size}=64; \texttt{batch\_size}=10; \texttt{nf}=64; \texttt{tf\_type}=partial; \texttt{training\_type}=inc; \texttt{seed}=0 \\
tiny & ERACECCLDC,tiny,m10000.yaml & ERACECCLDC & \texttt{optim}=AdamW; \texttt{learning\_rate}=0.0005; \texttt{momentum}=0; \texttt{weight\_decay}=0.0001; \texttt{img\_size}=64; \texttt{dim\_in}=2048; \texttt{n\_classes}=200; \texttt{n\_tasks}=100; \texttt{mem\_size}=10000; \texttt{mem\_batch\_size}=64; \texttt{batch\_size}=10; \texttt{nf}=64; \texttt{tf\_type}=partial; \texttt{training\_type}=inc; \texttt{seed}=0; \texttt{randaug\_m}=11; \texttt{randaug\_n}=1; \texttt{kd\_lambda}=1 \\
tiny & ERACECCLDC,tiny,m2000.yaml & ERACECCLDC & \texttt{optim}=AdamW; \texttt{learning\_rate}=0.0005; \texttt{momentum}=0; \texttt{weight\_decay}=0.0001; \texttt{img\_size}=64; \texttt{dim\_in}=2048; \texttt{n\_classes}=200; \texttt{n\_tasks}=100; \texttt{mem\_size}=2000; \texttt{mem\_batch\_size}=64; \texttt{batch\_size}=10; \texttt{nf}=64; \texttt{tf\_type}=partial; \texttt{training\_type}=inc; \texttt{seed}=0; \texttt{randaug\_m}=11; \texttt{randaug\_n}=1; \texttt{kd\_lambda}=1 \\
tiny & ERACECCLDC,tiny,m5000.yaml & ERACECCLDC & \texttt{optim}=AdamW; \texttt{learning\_rate}=0.0005; \texttt{momentum}=0; \texttt{weight\_decay}=0.0001; \texttt{img\_size}=64; \texttt{dim\_in}=2048; \texttt{n\_classes}=200; \texttt{n\_tasks}=100; \texttt{mem\_size}=5000; \texttt{mem\_batch\_size}=64; \texttt{batch\_size}=10; \texttt{nf}=64; \texttt{tf\_type}=partial; \texttt{training\_type}=inc; \texttt{seed}=0; \texttt{randaug\_m}=11; \texttt{randaug\_n}=1; \texttt{kd\_lambda}=1 \\
tiny & ERCCLDC,tiny,m10000.yaml & ERCCLDC & \texttt{optim}=AdamW; \texttt{learning\_rate}=0.0005; \texttt{momentum}=0; \texttt{weight\_decay}=0.0001; \texttt{img\_size}=64; \texttt{dim\_in}=2048; \texttt{n\_classes}=200; \texttt{n\_tasks}=100; \texttt{mem\_size}=10000; \texttt{mem\_batch\_size}=64; \texttt{batch\_size}=10; \texttt{nf}=64; \texttt{tf\_type}=full; \texttt{training\_type}=inc; \texttt{seed}=0; \texttt{randaug\_m}=11; \texttt{randaug\_n}=1; \texttt{kd\_lambda}=2 \\
tiny & ERCCLDC,tiny,m2000.yaml & ERCCLDC & \texttt{optim}=AdamW; \texttt{learning\_rate}=0.0005; \texttt{momentum}=0; \texttt{weight\_decay}=0.0001; \texttt{img\_size}=64; \texttt{dim\_in}=2048; \texttt{n\_classes}=200; \texttt{n\_tasks}=100; \texttt{mem\_size}=2000; \texttt{mem\_batch\_size}=64; \texttt{batch\_size}=10; \texttt{nf}=64; \texttt{tf\_type}=full; \texttt{training\_type}=inc; \texttt{seed}=0; \texttt{randaug\_m}=11; \texttt{randaug\_n}=1; \texttt{kd\_lambda}=2 \\
tiny & ERCCLDC,tiny,m5000.yaml & ERCCLDC & \texttt{optim}=AdamW; \texttt{learning\_rate}=0.0005; \texttt{momentum}=0; \texttt{weight\_decay}=0.0001; \texttt{img\_size}=64; \texttt{dim\_in}=2048; \texttt{n\_classes}=200; \texttt{n\_tasks}=100; \texttt{mem\_size}=5000; \texttt{mem\_batch\_size}=64; \texttt{batch\_size}=10; \texttt{nf}=64; \texttt{tf\_type}=full; \texttt{training\_type}=inc; \texttt{seed}=0; \texttt{randaug\_m}=11; \texttt{randaug\_n}=1; \texttt{kd\_lambda}=2 \\
tiny & GSA,tiny,m10000.yaml & GSA & \texttt{optim}=AdamW; \texttt{learning\_rate}=0.0005; \texttt{momentum}=0; \texttt{weight\_decay}=0.0001; \texttt{img\_size}=64; \texttt{dim\_in}=2048; \texttt{n\_classes}=200; \texttt{n\_tasks}=100; \texttt{mem\_size}=10000; \texttt{mem\_batch\_size}=64; \texttt{batch\_size}=10; \texttt{nf}=64; \texttt{tf\_type}=partial; \texttt{training\_type}=inc; \texttt{seed}=0 \\
tiny & GSA,tiny,m2000.yaml & GSA & \texttt{optim}=AdamW; \texttt{learning\_rate}=0.0005; \texttt{momentum}=0; \texttt{weight\_decay}=0.0001; \texttt{img\_size}=64; \texttt{dim\_in}=2048; \texttt{n\_classes}=200; \texttt{n\_tasks}=100; \texttt{mem\_size}=2000; \texttt{mem\_batch\_size}=64; \texttt{batch\_size}=10; \texttt{nf}=64; \texttt{tf\_type}=partial; \texttt{training\_type}=inc; \texttt{seed}=0 \\
tiny & GSA,tiny,m5000.yaml & GSA & \texttt{optim}=AdamW; \texttt{learning\_rate}=0.0005; \texttt{momentum}=0; \texttt{weight\_decay}=0.0001; \texttt{img\_size}=64; \texttt{dim\_in}=2048; \texttt{n\_classes}=200; \texttt{n\_tasks}=100; \texttt{mem\_size}=5000; \texttt{mem\_batch\_size}=64; \texttt{batch\_size}=10; \texttt{nf}=64; \texttt{tf\_type}=partial; \texttt{training\_type}=inc; \texttt{seed}=0 \\
tiny & GSACCLDC,tiny,m10000.yaml & GSACCLDC & \texttt{optim}=AdamW; \texttt{learning\_rate}=0.0005; \texttt{momentum}=0; \texttt{weight\_decay}=0.0001; \texttt{img\_size}=64; \texttt{dim\_in}=2048; \texttt{n\_classes}=200; \texttt{n\_tasks}=100; \texttt{mem\_size}=10000; \texttt{mem\_batch\_size}=64; \texttt{batch\_size}=10; \texttt{nf}=64; \texttt{tf\_type}=partial; \texttt{training\_type}=inc; \texttt{seed}=0; \texttt{randaug\_m}=11; \texttt{randaug\_n}=1 \\
tiny & GSACCLDC,tiny,m2000.yaml & GSACCLDC & \texttt{optim}=AdamW; \texttt{learning\_rate}=0.0005; \texttt{momentum}=0; \texttt{weight\_decay}=0.0001; \texttt{img\_size}=64; \texttt{dim\_in}=2048; \texttt{n\_classes}=200; \texttt{n\_tasks}=100; \texttt{mem\_size}=2000; \texttt{mem\_batch\_size}=64; \texttt{batch\_size}=10; \texttt{nf}=64; \texttt{tf\_type}=partial; \texttt{training\_type}=inc; \texttt{seed}=0; \texttt{randaug\_m}=11; \texttt{randaug\_n}=1 \\
tiny & GSACCLDC,tiny,m5000.yaml & GSACCLDC & \texttt{optim}=AdamW; \texttt{learning\_rate}=0.0005; \texttt{momentum}=0; \texttt{weight\_decay}=0.0001; \texttt{img\_size}=64; \texttt{dim\_in}=2048; \texttt{n\_classes}=200; \texttt{n\_tasks}=100; \texttt{mem\_size}=5000; \texttt{mem\_batch\_size}=64; \texttt{batch\_size}=10; \texttt{nf}=64; \texttt{tf\_type}=partial; \texttt{training\_type}=inc; \texttt{seed}=0; \texttt{randaug\_m}=11; \texttt{randaug\_n}=1 \\
tiny & OCM,tiny,m10000.yaml & OCM & \texttt{optim}=AdamW; \texttt{learning\_rate}=0.001; \texttt{momentum}=0; \texttt{weight\_decay}=0; \texttt{img\_size}=64; \texttt{dim\_in}=2048; \texttt{n\_classes}=200; \texttt{n\_tasks}=100; \texttt{mem\_size}=10000; \texttt{mem\_batch\_size}=64; \texttt{batch\_size}=10; \texttt{nf}=64; \texttt{tf\_type}=full; \texttt{training\_type}=inc; \texttt{seed}=0; \texttt{proj\_dim}=128 \\
tiny & OCM,tiny,m2000.yaml & OCM & \texttt{optim}=AdamW; \texttt{learning\_rate}=0.001; \texttt{momentum}=0; \texttt{weight\_decay}=0; \texttt{img\_size}=64; \texttt{dim\_in}=2048; \texttt{n\_classes}=200; \texttt{n\_tasks}=100; \texttt{mem\_size}=2000; \texttt{mem\_batch\_size}=64; \texttt{batch\_size}=10; \texttt{nf}=64; \texttt{tf\_type}=full; \texttt{training\_type}=inc; \texttt{seed}=0; \texttt{proj\_dim}=128 \\
tiny & OCM,tiny,m5000.yaml & OCM & \texttt{optim}=AdamW; \texttt{learning\_rate}=0.001; \texttt{momentum}=0; \texttt{weight\_decay}=0; \texttt{img\_size}=64; \texttt{dim\_in}=2048; \texttt{n\_classes}=200; \texttt{n\_tasks}=100; \texttt{mem\_size}=5000; \texttt{mem\_batch\_size}=64; \texttt{batch\_size}=10; \texttt{nf}=64; \texttt{tf\_type}=full; \texttt{training\_type}=inc; \texttt{seed}=0; \texttt{proj\_dim}=128 \\
tiny & OCMCCLDC,tiny,m10000.yaml & OCMCCLDC & \texttt{optim}=AdamW; \texttt{learning\_rate}=0.001; \texttt{momentum}=0; \texttt{weight\_decay}=0; \texttt{img\_size}=64; \texttt{dim\_in}=2048; \texttt{n\_classes}=200; \texttt{n\_tasks}=100; \texttt{mem\_size}=10000; \texttt{mem\_batch\_size}=64; \texttt{batch\_size}=10; \texttt{nf}=64; \texttt{tf\_type}=full; \texttt{training\_type}=inc; \texttt{seed}=0; \texttt{randaug\_m}=11; \texttt{randaug\_n}=1; \texttt{kd\_lambda}=4; \texttt{proj\_dim}=128 \\
tiny & OCMCCLDC,tiny,m2000.yaml & OCMCCLDC & \texttt{optim}=AdamW; \texttt{learning\_rate}=0.001; \texttt{momentum}=0; \texttt{weight\_decay}=0; \texttt{img\_size}=64; \texttt{dim\_in}=2048; \texttt{n\_classes}=200; \texttt{n\_tasks}=100; \texttt{mem\_size}=2000; \texttt{mem\_batch\_size}=64; \texttt{batch\_size}=10; \texttt{nf}=64; \texttt{tf\_type}=full; \texttt{training\_type}=inc; \texttt{seed}=0; \texttt{randaug\_m}=11; \texttt{randaug\_n}=1; \texttt{kd\_lambda}=4; \texttt{proj\_dim}=128 \\
tiny & OCMCCLDC,tiny,m5000.yaml & OCMCCLDC & \texttt{optim}=AdamW; \texttt{learning\_rate}=0.001; \texttt{momentum}=0; \texttt{weight\_decay}=0; \texttt{img\_size}=64; \texttt{dim\_in}=2048; \texttt{n\_classes}=200; \texttt{n\_tasks}=100; \texttt{mem\_size}=5000; \texttt{mem\_batch\_size}=64; \texttt{batch\_size}=10; \texttt{nf}=64; \texttt{tf\_type}=full; \texttt{training\_type}=inc; \texttt{seed}=0; \texttt{randaug\_m}=11; \texttt{randaug\_n}=1; \texttt{kd\_lambda}=4; \texttt{proj\_dim}=128 \\
tiny & ONPRO,tiny,m10000.yaml & OnPro & \texttt{optim}=AdamW; \texttt{learning\_rate}=0.0005; \texttt{momentum}=0; \texttt{weight\_decay}=0.0001; \texttt{img\_size}=64; \texttt{dim\_in}=2048; \texttt{n\_classes}=200; \texttt{n\_tasks}=100; \texttt{mem\_size}=10000; \texttt{mem\_batch\_size}=64; \texttt{batch\_size}=10; \texttt{nf}=64; \texttt{tf\_type}=full; \texttt{training\_type}=inc; \texttt{seed}=0 \\
tiny & ONPRO,tiny,m2000.yaml & OnPro & \texttt{optim}=AdamW; \texttt{learning\_rate}=0.0005; \texttt{momentum}=0; \texttt{weight\_decay}=0.0001; \texttt{img\_size}=64; \texttt{dim\_in}=2048; \texttt{n\_classes}=200; \texttt{n\_tasks}=100; \texttt{mem\_size}=2000; \texttt{mem\_batch\_size}=64; \texttt{batch\_size}=10; \texttt{nf}=64; \texttt{tf\_type}=full; \texttt{training\_type}=inc; \texttt{seed}=0 \\
tiny & ONPRO,tiny,m5000.yaml & OnPro & \texttt{optim}=AdamW; \texttt{learning\_rate}=0.0005; \texttt{momentum}=0; \texttt{weight\_decay}=0.0001; \texttt{img\_size}=64; \texttt{dim\_in}=2048; \texttt{n\_classes}=200; \texttt{n\_tasks}=100; \texttt{mem\_size}=5000; \texttt{mem\_batch\_size}=64; \texttt{batch\_size}=10; \texttt{nf}=64; \texttt{tf\_type}=full; \texttt{training\_type}=inc; \texttt{seed}=0 \\
tiny & ONPROCCLDC,tiny,m10000.yaml & OnProCCLDC & \texttt{optim}=AdamW; \texttt{learning\_rate}=0.0005; \texttt{momentum}=0; \texttt{weight\_decay}=0.0001; \texttt{img\_size}=64; \texttt{dim\_in}=2048; \texttt{n\_classes}=200; \texttt{n\_tasks}=100; \texttt{mem\_size}=10000; \texttt{mem\_batch\_size}=64; \texttt{batch\_size}=10; \texttt{nf}=64; \texttt{tf\_type}=full; \texttt{training\_type}=inc; \texttt{seed}=0; \texttt{randaug\_m}=11; \texttt{randaug\_n}=1 \\
tiny & ONPROCCLDC,tiny,m2000.yaml & OnProCCLDC & \texttt{optim}=AdamW; \texttt{learning\_rate}=0.0005; \texttt{momentum}=0; \texttt{weight\_decay}=0.0001; \texttt{img\_size}=64; \texttt{dim\_in}=2048; \texttt{n\_classes}=200; \texttt{n\_tasks}=100; \texttt{mem\_size}=2000; \texttt{mem\_batch\_size}=64; \texttt{batch\_size}=10; \texttt{nf}=64; \texttt{tf\_type}=full; \texttt{training\_type}=inc; \texttt{seed}=0; \texttt{randaug\_m}=11; \texttt{randaug\_n}=1 \\
tiny & ONPROCCLDC,tiny,m5000.yaml & OnProCCLDC & \texttt{optim}=AdamW; \texttt{learning\_rate}=0.0005; \texttt{momentum}=0; \texttt{weight\_decay}=0.0001; \texttt{img\_size}=64; \texttt{dim\_in}=2048; \texttt{n\_classes}=200; \texttt{n\_tasks}=100; \texttt{mem\_size}=5000; \texttt{mem\_batch\_size}=64; \texttt{batch\_size}=10; \texttt{nf}=64; \texttt{tf\_type}=full; \texttt{training\_type}=inc; \texttt{seed}=0; \texttt{randaug\_m}=11; \texttt{randaug\_n}=1 \\
\end{longtable}
\end{landscape}
